Can SOLARBURST go silicon? A systematic analysis on software supply chain attacks for VLSI design flows

An attacker targeting the software supply chain (SWSC) of VLSI tools can fully subvert the VLSI design pipeline through purely software level compromises. However, cur- rent literature on both SWSC and VLSI hardware security has not explored how software can be used to subvert the security of the VLSI design flow. In order to bridge this gap, this paper presents a systematic analysis of the vulnerable surface of VLSI from a SWSC standpoint. We carry this anal- ysis through three major activities. First, we did an empirical analysis of VLSI software suites, focusing on their software composition, security features, and tool interactions within the VLSI design flow. Second, we develop a VLSI-SWSC attack taxonomy model that links software supply chain at- tacks and their mechanisms to the VLSI attacks they enable, the design-flow stages they affect, and their resulting security outcomes, allowing us to identify 717 possible new attacks, including 60 high feasibility attacks supported by evidence collected in our empirical analysis. Third, we identify what possible security outcomes can be achieved by an attacker from these attacks and produce a comprehensive VLSI SWSC threat model. We evaluate the feasibility of the attacks identi- fied by our taxonomy across VLSI design stages and assess existing defenses to determine which attacks are mitigated and which remain unaddressed. In addition, we present case studies using a reference VLSI design flow consisting of open- source VLSI tools and highlight attacks identified through our taxonomy on the VLSI SWSC uniquely from a software perspective.

==> sections/security-outcomes.tex <==


We move to answer \textbf{RQ2:}``What are the potential security outcomes of SWSC attacks, and how can we systematically categorize categorize these outcomes to ensure a comprehensive and exhaustive security taxonomy?'', with the following sub-research questions, which are aligned to the CIA triad:\\
\textbf{RQ 2.1:} What are confidentiality-related outcomes with respect to tools' capabilities?\\
\textbf{RQ 2.2:} What are integrity-related outcomes with respect to tools' capabilities?\\
\textbf{RQ 2.3:} What are availability-related outcomes with respect to tools' capabilities?\\

%\begin{itemize}
 %   \item RQ 3.1: What are confidentiality related outcomes with respect to tools capabilities?
  %  \item RQ 3.2: What are Integrity related outcomes with respect to tools capabilities?
   % \item RQ 3.3: What are availability related outcomes with respect to tools capabilities?
%\end{itemize}

To systematically answer the research question, we identified the attack surface across the VLSI design processes by focusing on confidentiality (or privacy), integrity, and availability outcomes. These outcomes were then instantiated at each stage of our design and across the tool flow we studied. With this, we produced a structured representation of potential attack possibilities at each stage of the VLSI design process. 
%These attack trees are further explored with respect to their attacks feasibility and impact, attack surface and risk surface. 

\subsection{Attack Classes}
\label{subsec:attacks}

%\subhav{"was done by doing" :P} \fabiha{RESOLVED}

We constructed these trees through empirical analysis of VLSI software suites with respect to their vulnerabilities. Following is the detailed description of each tree.\\
\textbf{RQ 2.1: Confidentiality Attack Classes:}
We consider confidentiality attack classes within our threat surface. These include the protection of intellectual property (IP) (e.g., design netlists), design logic (e.g., gate-level/RTL design), and manufacturing details that, if exposed, could lead to IP theft or reverse engineering. Figure~\ref{AttackTrees} outlines the attack paths. CA1 targets IP theft: CA1T1 uses backdoored tools to extract RTL/netlists, while CA1T2 embeds scripts to exfiltrate design artifacts.\\

\begin{figure}[b]
  \centering
  \includegraphics[width=0.4\textwidth]{sections/Images/AttackTreesFinalFix.drawio.png}
  \caption{CIA-based attack tress for VLSI SWSC threats}
  \label{AttackTrees}
  %\subhav{s/Trojanize/Trojanized/}
\end{figure}

%\begin{figure}
 %   \centering
  %  \includegraphics[width=0.7\linewidth]{sections/Images/Blank diagram (2).png}
   % \caption{Confidentiality Attack Tree}
    %\label{confidentialitry}
%\end{figure}
%Confidentiality refers to the protection of sensitive information from unauthorized access or disclosure. In the VLSI design process, this includes safeguarding intellectual property (IP) (design net-lists), design logic (e.g., gate-level or RTL design), and other manufacturing details that, if exposed, could lead to IP theft, or reverse engineering. Potential security outcomes from confidentiality breaches can vary based on the type of tool compromised as well as at what step of VLSI software supply chain that tool has been compromised. 
%Figure~\ref{confidentialitry} shows the attack tree of potential paths to compromise the confidentiality on any step of VLSI design process.
%CA1 focuses on stealing critical data like RTL code, netlists, and blueprints. CA1T1 involves distributing compromised EDA tools with backdoors to extract sensitive design data during stages like RTL synthesis and placement. CA1T2 targets automation by embedding malicious flow scripts that exfiltrate design files, IP cores and netlists. 
\textbf{RQ 2.2: Integrity Attack Classes:}
Supply chain attacks can compromise the integrity of VLSI software by introducing malicious modifications, reducing reliability, or causing design failures 
%\subhav{"Supply chain attacks can compromise the integrity of VLSI software by introducing malicious modifications, reducing reliability, or causing design failures."\fabiha{RESOLVED}?}
IA1 targets design trojanization (i.e., inserting a malicious element in the design). 
Figure~\ref{AttackTrees} presents the integrity attack tree. IA1 targets design Trojans. 
IA1T1: \textit{Trojan Insertion via compromised tools or artifacts} --- e.g., using a modified Yosys binary to inject logic at synthesis. 
IA1T2: \textit{Verification bypass for Trojan persistence} --- e.g., hooking SymbiYosys to suppress assertion failures. 
IA2 focuses on faulty outputs. 
IA2T1: \textit{Test degradation or design corruption} --- e.g., flow scripts in OpenTimer or ABC that masks timing violations or break circuit connectivity.\\
%Figure~\ref{intergrity} illustrates the integrity attack tree, highlighting methods to compromise the integrity of the VLSI design. IA1 focuses on Trojanizing the design, where malicious elements are embedded into the circuit to introduce vulnerabilities. IA1T1 involves inserting Trojans through malicious EDA tools or by distributing compromised input artifacts. IA1T2 ensures that Trojans remain undetected during testing or verification, allowing them to persist into production. IA2 targets the production of unavailable designs by leveraging EDA tools or flow scripts to introduce flaws, hinder testing capabilities, or create designs that are nonfunctional under specific conditions.
%\begin{figure}
 %   \centering
  %  \includegraphics[width=0.7\linewidth]{sections/Images/Blank diagram (15).png}
   % \caption{Integrity Attack Tree}
    %\label{intergrity}
%\end{figure}
\textbf{RQ 2.3: Availability Attack Classes:}
Availability attacks hinder tool or flow execution (Figure~\ref{AttackTrees}). 
This includes attacks such as AA1T1: \textit{Malicious input slows tools} — e.g., OpenSTA with malformed timing files. 
AA1T2: \textit{Overloaded binaries} — e.g., Yosys with delay-introducing hooks. 
AA2T1: \textit{Inefficient scripts} — e.g., TCL loops in Magic. 
AA2T2: \textit{Crash-inducing inputs} — e.g., oversized BLIF in ABC.\\
%Availability attacks disrupt or degrade the performance of tools, scripts, or workflows in the VLSI design process. Figure~\ref{availability} illustrates the attack tree for availability. AA1 focuses on degrading the performance of the EDA tool through malicious input artifacts (AA1T1) or poorly performing tools (AA1T2). AA2 targets flow performance by distributing suboptimal flow scripts (AA2T1) or manipulating input artifacts to hinder workflows (AA2T2).

%\subhav{I'm not sure I understand the difference between AA1 and AA2. What's the difference between "EDA tool performance" and "flow performance"? Is that during synthesis vs when a user is using the tool?}

%\begin{figure}
 %   \centering
  %  \includegraphics[width=1.0\linewidth]{sections/Images/Blank diagram (5).png}
  %  \caption{Availability Attack Tree}
   % \label{availability}
%\end{figure}



\subsection{Security Outcomes: Feasibility, Impact, Risk}

%\subhav{I think "security outcome" is awkward wording -- that sounds like something is being secured. (Sorry I didn't mention this earlier about the abstract.) Could it be just "outcomes" or "security implications".}

Beyond categorization, we also rate these attack classes in terms of feasibility, attack surface, and risk, as detailed below. \\
\textbf{Attack Surface (Libraries):}
We then combine the information identified earlier regarding open source software composition, and use it provide perspective on the potential attack surface for each individual component explored.
In short, the tools presented all show varied composition of open source components and functions, leading to varying degrees of compromise and with different impacts.
%This part of the taxonomy provides a holistic overview of disclosed and undisclosed dependencies of tools at each step of the VLSI design process. 
The attack surface analysis highlights that open-source tools like Yosys (21), Magic (19), OpenSTA (23), and OpenRoad (38) show transparency by disclosing dependencies but rely on open-source maintainers.
For example, a tool as Yosys, depends on more than 1433 maintainers through its dependencies (dynamic and static).
The dependencies would allow a rogue upstream maintainer to modify Yosys's behavior by injecting a command during its execution. \\
%\subhav{"Yosys's behavior"?} \fabiha{Resolved} \\
%In contrast, commercial tools like Cadence Genus, VCS, and ModelSim disclose no dependencies, limiting visibility into their components.
\textbf{Risk Surface (Vulnerabilities):}
Similarly, we can gauge the relative risk is derived from these dependencies.
Given that these tools expose open source libraries during their operations, an attacker can use this information to subvert their execution.\\
For this, we collected CVE information for components and dependencies, and identified critical dependencies within it.\\
We also show the results on Table~\ref{tab:shared_static_tpl}, where we display that most libraries are historically affected by one severe (i.e., CVSS greater than 7.5) somewhere in its dependency chain.\\ 
%\subhav{"one severe CVE"?} \fabiha{RESOLVED} \subhav{??}
The highest number of CVEs are associated with libexpat (14 in total), which is found in Yosys and OpenLane, with severity scores reaching up to 9.8. 
These CVEs allow attackers to carry out Integer Overflows (which may lead to arbitrary code execution (CVE-2023-43787), or Infinite Loop leading to denial of service conditions (CVE-2023-43786), and out-of-bounds read errors allowing unauthorized access to system memory (CVE-2023-43785).\\ 
\textbf{Feasibility and Impact:}
These categorization also allows us to understand how likely is an attacker to succeed when carrying out attacks on this SWSC.\\
Concretely, we identify that attackers on tools further down the line are either \emph{modifying steps} (i.e., those that may change the eventual design), or \emph{gating steps} (i.e,. those who could be used to detect a modified design).
We measure \emph{feasibility} as both the likelihood of an exploitable vulnerability existing, with the likelihood of it being detected.\\
The former is related to Risk and Attack surface outlined above, whereas the latter is defined by its position in the pipeline. That is, if there are gating steps further down the line, an attacker would also require to compromise those steps to avoid detection.






%The confidentiality security outcomes in the VLSI design process, as outlined in the confidentiality attack tree, vary in feasibility and impact across different stages. 
%High-risk stages, such as High-Level Synthesis, Logic Synthesis, and Placement and Routing, are particularly vulnerable to attacks like the distribution of backdoored EDA tools (CA1T1) and malicious flowscripts (CA1T2), with both showing high feasibility and impact. 
%These stages involve processing and transforming sensitive data, including RTL designs, netlists, and physical layouts, making them critical targets for attackers. 
%Conversely, steps like Fabrication demonstrate lower applicability to confidentiality risks due to limited automation and direct tool involvement.
%
%The integrity attack tree shows the insertion of Trojan via backdoored EDA tools (IA1T1), compromising the input artifacts (IA1T2), and malicious flow scripts (IA1T3), with varying feasibility and impact across the VLSI design process. 
%In specifications (Step 1), attacks like Trojanized templates (IA1T2) have moderate feasibility, introducing flaws into downstream design processes. 
%However, flow-scripts (IA1T3) have backdoored tools (IA1t1) have low feasibility due to limited reliance on automation at this stage. 
%In high level synthesis (Step 2), Trojanized EDA tools (IA1T1) can insert malicious logic into RTL designs, while compromised input constraints (IA1T2) introduce vulnerabilities. 
%Malicious flowscripts (IA1T3) automate synthesis tasks to manipulate design output, all with high feasibility and impact. 
%During verification (Step 3), backdoored tools (IA1T1) skew testing accuracy, and Trojanized test benches (IA1T2) which effects validation. 
%Malicious flowscripts (IA1T3) manipulates test coverage metrics, creating undetected vulnerabilities, with high feasibility and isgnificant impact on design correctness. 
%In logic synthesis (Step 4) and palcement and routing (Step 7), Trojanized tools (IA1T1) inject malicious routing paths or logic, while compromised constraints (IA1T2) degrade output quality. 
%For example, malicious flowscripts (IA1T3) in P\& R can alter physical layouts, impacting performance and reliability. 
%In static timing analysis (Step 8) and physical verification (Step 9), Trojanized EDA tools (IA1T1) have moderate feasibility and medium impact by manipulating timing reports or verification results, potentially masking critical violations. 
%Trojanized rule sets (IA1T2) have moderate feasibility and medium impact, as they degrade compliance checks like DRC or LVS, leading to incomplete design validation. 
%Malicious flowscripts (IA1T3) exhibit high feasibility and high impact by misrepresenting timing data or altering physical verification outputs, resulting in flawed manufacturing-ready designs. 
%For instance, a malicious script may approve a non-compliant layout for fabrication. In post design stages like fabrication (Step 10) and manufacturing testing (Step 12), Trojanized test patterns (IA1T2) have moderate feasibility and medium impact, as they hinder defect detection by compromising test coverage. 
%Malicious flowscripts (IA1T3), with low feasibility and minimal impact during fabrication, become highly feasible and highly impactful during manufacturing testing by skewing test outcomes or masking defects. 
%For example, in post silicon validation  (Step 11), malicious flowscripts (IA1T3) exhibit high feasibility and high impact, bypassing crucial validation checks and allowing flawed chips to proceed into production, significantly compromising product reliability. 
%
%The availability attack tree highlights potential availability attacks across the VLSI design process. 
%In specification phase (Step 1), availability risks are minimal as EDA tools, input artifacts, and flowscripts are rarely utilized  
%(low feasibility and impact). 
%However, during high level synthesis (Step 2), maliciously altered input artifacts (AA1T1, AA2T2) or poor performing tools (AA1T2) can significantly delay synthesis, with high feasibility and impact. 
%Similarly, in Verification (Step 3), poor test patterns (AA1T1) or malicious flowscripts (AA2T1) can disrupt simulations, leading to delays. 
%For Logic Synthesis (Step 4) and Post Synthesis Verification (Step 5), malicious artifacts and scripts (AA1T1, AA2T1) degrade tool efficiency and slow testing processes, exhibiting high feasibility and impact. 
%During Design for Testability (Step 6), poor performing tools and flowscripts (AA1T2, AA2T1) can hinder test structure developmnet. 
%In Placement and Routing (Step 7) and Static Timing Analysis (Step 8), flowscripts (AA2T1) and faulty constraints (AA2T2) delay optimization and timing closure (moderate to high impact). 
%For Physical Verification (Step 9), manipulated rule sets (AA2T2) and malicious scripts (AA2T1) affect compliance checks, with high feasibility and impact. 
%Fabrication (Step 10) sees limited disruption potential due to minimal reliance on EDA tools. 
%However, in Post-Silicon Validation (Step 11) and Manufacturing Testing (Step 12), faulty input patterns (AA1T1) or malicious scripts (AA2T1) directly hinder validation and throughput, leading to high delays and compromised product readiness. 


%Further, the library glibc, also found in Yosys, OpenRoad, Magic, and ABC, is associated with vulnerabilities such as code execution with elevated privileges via crafted environment variables (CVE-2023-4911, CVE Score: 7.8, High) and use-after-free errors causing application crashes (CVE-2023-4813 and CVE-2023-4806, CVE Score: 5.9, Medium). Another library filesystem, present in Yosys, OpenRoad, Magic, and ABC, is associated with vulnerabilities including data leakage by reading unintended data from deleted files on an msdosfs filesystem (CVE-2023-5368, CVE Score: 6.5, Medium) and unauthorized file system actions through CSRF attacks, potentially allowing web shell uploads (CVE-2023-4827, CVE Score: 8.8, High).















